A Cross-Platform Collection of Social Network Profiles

The proliferation of Internet-enabled devices and services has led to a shifting balance between digital and analogue aspects of our everyday lives. In the face of this development there is a growing demand for the study of privacy hazards, the potential for unique user de-anonymization and information leakage between the various social media profiles many of us maintain. To enable the structured study of such adversarial effects, this paper presents a dedicated dataset of cross-platform social network personas (i.e., the same person has accounts on multiple platforms). The corpus comprises 850 users who generate predominantly English content. Each user object contains the online footprint of the same person in three distinct social networks: Twitter, Instagram and Foursquare. In total, it encompasses over 2.5M tweets, 340k check-ins and 42k Instagram posts. We describe the collection methodology, characteristics of the dataset, and how to obtain it. Finally, we discuss a common use case, cross-platform user identification.

==> code.tex <==
\section{Code}
\label{sec:code}
How the dataset looks like?

The format of the data set is the following.

For each user, there are three objects. We only release the ids of content.

? dataset scheme? 

Twitter user_id - Tweet ids
Instagram user_id - Instagram ids
Foursquare venue_id and tweet id associated


\begin{table}
\centering
\caption{Frequency of Special Characters}
\begin{tabular}{|c|c|l|} \hline
Non-English or Math&Frequency&Comments\\ \hline
\O & 1 in 1,000& For Swedish names\\ \hline
$\pi$ & 1 in 5& Common in math\\ \hline
\$ & 4 in 5 & Used in business\\ \hline
$\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
\hline\end{tabular}
\end{table}



The reason why the content from Foursquare is presented this way is because the \emph{user_id} is not publicly accessible through the API.

How do people use the dataset?

In the following repo we provide scripts which assemble, with minimal effort, the data set given an appropriate API id and key.

? Include small tutorial?
